Demystifying the Base and Novel Performances for Few-shot Class-incremental Learning

Few-shot class-incremental learning (FSCIL) has addressed challenging real-world scenarios where unseen novel classes continually arrive with few samples. In these scenarios, it is required to develop a model that recognizes the novel classes without forgetting prior knowledge. In other words, FSCIL aims to maintain the base performance and improve the novel performance simultaneously. However, there is little study to investigate the two performances separately. In this paper, we first decompose the entire model into four types of parameters and demonstrate that the tendency of the two performances varies greatly with the updated parameters when the novel classes appear. Based on the analysis, we propose a simple method for FSCIL, coined as NoNPC, which uses normalized prototype classifiers without further training for incremental novel classes. It is shown that our straightforward method has comparable performance with the sophisticated state-of-the-art algorithms.

==> table/cifar_clipping_perf.tex <==
\begin{table}[t]
\footnotesize
    \centering
    \caption{Base, novel, and weighted performance of updating only $h_i$ according to the clipping norm.}\label{tab:cifar_norm}
    \begin{tabular}{ccccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Performance} & \multirow{2}{*}{\vspace{-3pt}Norm} & \multicolumn{9}{c}{Session} \\
    \cmidrule{3-11}
    & & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
    \midrule
    \multirow{4}{*}{Base}     & 1.0  & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
                              & 2.5  & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
                              & 5.0  & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
                              & -    & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \midrule
    \multirow{4}{*}{Novel}    & 1.0  & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
                              & 2.5  & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
                              & 5.0  & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
                              & -    & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \midrule
    \multirow{4}{*}{Weighted} & 1.0  & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
                              & 2.5  & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
                              & 5.0  & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
                              & -    & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \bottomrule
    \end{tabular}
\end{table}

==> table/cifar_cosine_decomp_perf.tex <==
\begin{table}[t]
\footnotesize
    \centering
    \caption{With cosine classifier, Base, novel, and weighted performance according to the update parts during novel sessions on CIFAR100. Decomposed parameters are described in Table~\ref{tab:notation}.}\label{tab:cifar_decomp_w_cosine_cls}
    \vspace{-5pt}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cc|cccc|ccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Performance} & \multirow{2}{*}{\vspace{-3pt}Model} & \multicolumn{4}{c|}{Update parts} & \multicolumn{9}{c}{Session} \\
    \cmidrule{3-15}
    & & $f$ & $h_0$ & $h_{-i}$ & $h_i$ & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
    \midrule
    \multirow{5}{*}{Base} & M1 &  &  &  &                    & 73.47 & 73.47 & 73.47 & 73.47 & 73.47 & 73.47 & 73.47 & 73.47 & 73.47 \\
    & M2 & &  &  & \checkmark                                & 73.47 & 51.80 & 45.93 & 40.05 & 35.12 & 29.98 & 27.93 & 26.07 & 22.70 \\
    & M3 & &  & \checkmark & \checkmark                      & 73.47 & 51.80 & 57.68 & 56.18 & 54.37 & 51.78 & 53.93 & 52.98 & 49.27 \\
    & M4 & & \checkmark & \checkmark & \checkmark            & 73.47 & 56.20 & 54.43 & 51.90 & 48.43 & 43.83 & 43.55 & 43.03 & 38.08 \\
    & M5 & \checkmark & \checkmark & \checkmark & \checkmark & 73.47 & 46.92 & 29.00 & 20.47 & 13.68 & 11.32 & 7.93 & 6.58 & 3.42 \\
    \midrule
    \multirow{5}{*}{Novel} & M1 & &  &  &                    & - & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & M2 & &  &  & \checkmark                                & - & 73.80 & 55.90 & 37.53 & 29.20 & 27.92 & 26.10 & 23.09 & 24.57 \\
    & M3 & &  & \checkmark & \checkmark                      & - & 73.80 & 30.50 & 19.93 & 14.25 & 15.28 & 11.00 & 10.09 & 9.65 \\
    & M4 & & \checkmark & \checkmark & \checkmark            & - & 72.40 & 31.90 & 23.47 & 16.45 & 17.24 & 12.23 & 12.14 & 10.50 \\
    & M5 & \checkmark & \checkmark & \checkmark & \checkmark & - & 57.00 & 27.80 & 23.27 & 13.75 & 13.88 & 11.10 & 9.46 & 7.95 \\
    \midrule
    \multirow{5}{*}{Weighted} & M1 & &  &  &                 & 73.47 & 67.82 & 62.97 & 58.77 & 55.10 & 51.86 & 48.98 & 46.40 & 44.08 \\
    & M2 & &  &  & \checkmark                                & 73.47 & 53.49 & 47.36 & 39.55 & 33.64 & 29.38 & 27.32 & 24.97 & 23.45 \\
    & M3 & &  & \checkmark & \checkmark                      & 73.47 & 53.49 & 53.80 & 48.93 & 44.34 & 41.05 & 39.62 & 37.18 & 33.42 \\
    & M4 & & \checkmark & \checkmark & \checkmark            & 73.47 & 57.45 & 51.21 & 46.21 & 40.44 & 36.01 & 33.11 & 31.65 & 27.05 \\
    & M5 & \checkmark & \checkmark & \checkmark & \checkmark & 73.47 & 47.69 & 28.83 & 21.03 & 13.70 & 12.07 & 8.99 & 7.64 & 5.23 \\
    \bottomrule
    \end{tabular}
    }
\end{table}

% \begin{table}[t]
% \footnotesize
%     \centering
%     \caption{Base, novel, and weighted performance according to the update parts during novel sessions on CIFAR100. Decomposed parameters are described in Table~\ref{tab:notation}.}\label{tab:cifar_decomp}
%     \vspace{-5pt}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{c|cccc|ccccccccc}
%     \toprule
%     \multirow{2}{*}{\vspace{-3pt}Performance} & \multicolumn{4}{c|}{Update parts} & \multicolumn{9}{c}{Session} \\
%     \cmidrule{2-14}
%     & $f$ & $h_0$ & $h_{-i}$ & $h_i$ & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
%     \midrule
%     \multirow{5}{*}{Base} &  &  &  &                    & 65.93 & 65.93 & 65.93 & 65.93 & 65.93 & 65.93 & 65.93 & 65.93 & 65.93 \\
%     &  &  &  & \checkmark                               & 65.93 & 54.77 & 49.13 & 44.10 & 41.92 & 37.40 & 36.07 & 34.23 & 29.87 \\
%     &  &  & \checkmark & \checkmark                     & 65.93 & 54.77 & 54.70 & 53.20 & 54.20 & 50.23 & 54.30 & 51.63 & 50.45 \\
%     &  & \checkmark & \checkmark & \checkmark           & 65.93 & 52.78 & 49.52 & 47.18 & 45.08 & 39.42 & 41.70 & 37.33 & 34.10 \\
%     % & \checkmark &  &  & \checkmark                     & 65.93 & 41.98 & 26.57 & 19.17 & 15.48 & 9.80 & 8.70 & 4.92 & 3.68 \\
%     % & \checkmark &  & \checkmark & \checkmark           & 65.93 & 42.10 & 28.88 & 20.15 & 15.78 & 11.70 & 5.60 & 6.47 & 4.72 \\
%     & \checkmark & \checkmark & \checkmark & \checkmark & 65.93 & 41.62 & 28.63 & 20.47 & 15.27 & 9.50 & 6.97 & 4.47 & 4.78 \\
%     \midrule
%     \multirow{5}{*}{Novel} &  &  &  &                   & -     & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%     &  &  &  & \checkmark                               & -     & 65.00 & 53.00 & 42.07 & 36.85 & 37.84 & 36.13 & 32.43 & 32.62 \\
%     &  &  & \checkmark & \checkmark                     & -     & 65.00 & 36.10 & 26.27 & 18.00 & 17.80 & 13.90 & 11.57 & 12.95 \\
%     &  & \checkmark & \checkmark & \checkmark           & -     & 67.40 & 40.70 & 30.93 & 22.20 & 21.60 & 17.47 & 14.00 & 15.52 \\
%     % & \checkmark &  &  & \checkmark                     & -     & 69.60 & 40.10 & 35.07 & 23.90 & 21.04 & 19.13 & 18.23 & 15.40 \\
%     % & \checkmark &  & \checkmark & \checkmark           & -     & 68.60 & 33.40 & 28.40 & 15.35 & 14.64 & 11.43 & 10.80 & 10.20 \\
%     & \checkmark & \checkmark & \checkmark & \checkmark & -     & 73.80 & 33.40 & 27.20 & 14.80 & 13.28 & 11.23 & 10.66 & 10.12 \\
%     \midrule
%     \multirow{5}{*}{Weighted} &  &  &  &                & 65.93 & 60.86 & 56.51 & 52.75 & 49.45 & 46.54 & 43.96 & 41.64 & 39.56 \\
%     &  &  &  & \checkmark                               & 65.93 & 55.55 & 49.69 & 43.69 & 40.65 & 37.53 & 36.09 & 33.57 & 30.97 \\
%     &  &  & \checkmark & \checkmark                     & 65.93 & 55.55 & 52.04 & 47.81 & 45.15 & 40.69 & 40.83 & 36.87 & 35.45 \\
%     &  & \checkmark & \checkmark & \checkmark           & 65.93 & 53.91 & 48.26 & 43.93 & 39.36 & 34.18 & 33.62 & 28.74 & 26.67 \\
%     % & \checkmark &  &  & \checkmark                     & 65.93 & 44.11 & 28.50 & 22.35 & 17.59 & 13.11 & 12.18 & 9.82 & 8.37 \\
%     % & \checkmark &  & \checkmark & \checkmark           & 65.93 & 44.14 & 29.53 & 21.80 & 15.67 & 12.56 & 7.54 & 8.06 & 6.91 \\
%     & \checkmark & \checkmark & \checkmark & \checkmark & 65.93 & 44.09 & 29.31 & 21.81 & 15.15 & 10.61 & 8.39 & 6.75 & 6.92 \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{table}

==> table/cifar_decomp_perf.tex <==
\begin{table}[h]
\footnotesize
    \centering
    \caption{Base, novel, and weighted performance according to the update parts during novel sessions on CIFAR100. Decomposed parameters are described in Table~\ref{tab:notation}.}\label{tab:cifar_decomp}
    \vspace{-5pt}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cc|cccc|ccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Performance} & \multirow{2}{*}{\vspace{-3pt}Model} & \multicolumn{4}{c|}{Update parts} & \multicolumn{9}{c}{Session} \\
    \cmidrule{3-15}
    & & $f$ & $h_0$ & $h_{-i}$ & $h_i$ & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
    \midrule
    \multirow{5}{*}{Base} & M1 &  &  &  &                    & 73.47 & 73.47 & 73.47 & 73.47 & 73.47 & 73.47 & 73.47 & 73.47 & 73.47 \\
    & M2 & &  &  & \checkmark                                & 73.47 & 51.80 & 45.93 & 40.05 & 35.12 & 29.98 & 27.93 & 26.07 & 22.70 \\
    & M3 & &  & \checkmark & \checkmark                      & 73.47 & 51.80 & 57.68 & 56.18 & 54.37 & 51.78 & 53.93 & 52.98 & 49.27 \\
    & M4 & & \checkmark & \checkmark & \checkmark            & 73.47 & 56.20 & 54.43 & 51.90 & 48.43 & 43.83 & 43.55 & 43.03 & 38.08 \\
    & M5 & \checkmark & \checkmark & \checkmark & \checkmark & 73.47 & 46.92 & 29.00 & 20.47 & 13.68 & 11.32 & 7.93 & 6.58 & 3.42 \\
    \midrule
    \multirow{5}{*}{Novel} & M1 & &  &  &                    & - & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    & M2 & &  &  & \checkmark                                & - & 73.80 & 55.90 & 37.53 & 29.20 & 27.92 & 26.10 & 23.09 & 24.57 \\
    & M3 & &  & \checkmark & \checkmark                      & - & 73.80 & 30.50 & 19.93 & 14.25 & 15.28 & 11.00 & 10.09 & 9.65 \\
    & M4 & & \checkmark & \checkmark & \checkmark            & - & 72.40 & 31.90 & 23.47 & 16.45 & 17.24 & 12.23 & 12.14 & 10.50 \\
    & M5 & \checkmark & \checkmark & \checkmark & \checkmark & - & 57.00 & 27.80 & 23.27 & 13.75 & 13.88 & 11.10 & 9.46 & 7.95 \\
    \midrule
    \multirow{5}{*}{Weighted} & M1 & &  &  &                 & 73.47 & 67.82 & 62.97 & 58.77 & 55.10 & 51.86 & 48.98 & 46.40 & 44.08 \\
    & M2 & &  &  & \checkmark                                & 73.47 & 53.49 & 47.36 & 39.55 & 33.64 & 29.38 & 27.32 & 24.97 & 23.45 \\
    & M3 & &  & \checkmark & \checkmark                      & 73.47 & 53.49 & 53.80 & 48.93 & 44.34 & 41.05 & 39.62 & 37.18 & 33.42 \\
    & M4 & & \checkmark & \checkmark & \checkmark            & 73.47 & 57.45 & 51.21 & 46.21 & 40.44 & 36.01 & 33.11 & 31.65 & 27.05 \\
    & M5 & \checkmark & \checkmark & \checkmark & \checkmark & 73.47 & 47.69 & 28.83 & 21.03 & 13.70 & 12.07 & 8.99 & 7.64 & 5.23 \\
    \bottomrule
    \end{tabular}
    }
\end{table}

% \begin{table}[t]
% \footnotesize
%     \centering
%     \caption{Base, novel, and weighted performance according to the update parts during novel sessions on CIFAR100. Decomposed parameters are described in Table~\ref{tab:notation}.}\label{tab:cifar_decomp}
%     \vspace{-5pt}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{c|cccc|ccccccccc}
%     \toprule
%     \multirow{2}{*}{\vspace{-3pt}Performance} & \multicolumn{4}{c|}{Update parts} & \multicolumn{9}{c}{Session} \\
%     \cmidrule{2-14}
%     & $f$ & $h_0$ & $h_{-i}$ & $h_i$ & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
%     \midrule
%     \multirow{5}{*}{Base} &  &  &  &                    & 65.93 & 65.93 & 65.93 & 65.93 & 65.93 & 65.93 & 65.93 & 65.93 & 65.93 \\
%     &  &  &  & \checkmark                               & 65.93 & 54.77 & 49.13 & 44.10 & 41.92 & 37.40 & 36.07 & 34.23 & 29.87 \\
%     &  &  & \checkmark & \checkmark                     & 65.93 & 54.77 & 54.70 & 53.20 & 54.20 & 50.23 & 54.30 & 51.63 & 50.45 \\
%     &  & \checkmark & \checkmark & \checkmark           & 65.93 & 52.78 & 49.52 & 47.18 & 45.08 & 39.42 & 41.70 & 37.33 & 34.10 \\
%     % & \checkmark &  &  & \checkmark                     & 65.93 & 41.98 & 26.57 & 19.17 & 15.48 & 9.80 & 8.70 & 4.92 & 3.68 \\
%     % & \checkmark &  & \checkmark & \checkmark           & 65.93 & 42.10 & 28.88 & 20.15 & 15.78 & 11.70 & 5.60 & 6.47 & 4.72 \\
%     & \checkmark & \checkmark & \checkmark & \checkmark & 65.93 & 41.62 & 28.63 & 20.47 & 15.27 & 9.50 & 6.97 & 4.47 & 4.78 \\
%     \midrule
%     \multirow{5}{*}{Novel} &  &  &  &                   & -     & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%     &  &  &  & \checkmark                               & -     & 65.00 & 53.00 & 42.07 & 36.85 & 37.84 & 36.13 & 32.43 & 32.62 \\
%     &  &  & \checkmark & \checkmark                     & -     & 65.00 & 36.10 & 26.27 & 18.00 & 17.80 & 13.90 & 11.57 & 12.95 \\
%     &  & \checkmark & \checkmark & \checkmark           & -     & 67.40 & 40.70 & 30.93 & 22.20 & 21.60 & 17.47 & 14.00 & 15.52 \\
%     % & \checkmark &  &  & \checkmark                     & -     & 69.60 & 40.10 & 35.07 & 23.90 & 21.04 & 19.13 & 18.23 & 15.40 \\
%     % & \checkmark &  & \checkmark & \checkmark           & -     & 68.60 & 33.40 & 28.40 & 15.35 & 14.64 & 11.43 & 10.80 & 10.20 \\
%     & \checkmark & \checkmark & \checkmark & \checkmark & -     & 73.80 & 33.40 & 27.20 & 14.80 & 13.28 & 11.23 & 10.66 & 10.12 \\
%     \midrule
%     \multirow{5}{*}{Weighted} &  &  &  &                & 65.93 & 60.86 & 56.51 & 52.75 & 49.45 & 46.54 & 43.96 & 41.64 & 39.56 \\
%     &  &  &  & \checkmark                               & 65.93 & 55.55 & 49.69 & 43.69 & 40.65 & 37.53 & 36.09 & 33.57 & 30.97 \\
%     &  &  & \checkmark & \checkmark                     & 65.93 & 55.55 & 52.04 & 47.81 & 45.15 & 40.69 & 40.83 & 36.87 & 35.45 \\
%     &  & \checkmark & \checkmark & \checkmark           & 65.93 & 53.91 & 48.26 & 43.93 & 39.36 & 34.18 & 33.62 & 28.74 & 26.67 \\
%     % & \checkmark &  &  & \checkmark                     & 65.93 & 44.11 & 28.50 & 22.35 & 17.59 & 13.11 & 12.18 & 9.82 & 8.37 \\
%     % & \checkmark &  & \checkmark & \checkmark           & 65.93 & 44.14 & 29.53 & 21.80 & 15.67 & 12.56 & 7.54 & 8.06 & 6.91 \\
%     & \checkmark & \checkmark & \checkmark & \checkmark & 65.93 & 44.09 & 29.31 & 21.81 & 15.15 & 10.61 & 8.39 & 6.75 & 6.92 \\
%     \bottomrule
%     \end{tabular}
%     }
% \end{table}

==> table/cifar_existing_perf.tex <==
\begin{table}[t]
\footnotesize
    \centering
    \caption{Base, novel, and weighted performance of existing algorithms on CIFAR100. B, N, and W indicate base, novel, and weighted performance, respectively.}\label{tab:cifar_existing}
    \begin{tabular}{cc|ccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Algorithm} & \multirow{2}{*}{\vspace{-3pt}Perf.} & \multicolumn{9}{c}{Session} \\
    \cmidrule{3-11}
    & & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
    \midrule
    \multirow{3}{*}{Base Model (XXXX)} & B & 72.93 & 63.83 & 60.52 & 57.47 & 55.62 & 51.97 & 49.83 & 49.42 & 44.02 \\
    & N & - & 57.40 & 42.60 & 35.73 & 31.05 & 30.40 & 29.03 & 26.31 & 28.12 \\
    & W & 72.93 & 63.34 & 57.96 & 53.12 & 49.47 & 45.62 & 42.90 & 40.91 & 37.66 \\
    \midrule
    \multirow{3}{*}{TOPIC~(\citeyear{tao2020few})} & B & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & N & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & W & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \midrule
    \multirow{3}{*}{F2M~(\citeyear{shi2021overcoming})} & B & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & N & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & W & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \midrule
    \multirow{3}{*}{CEC~(\citeyear{zhang2021few})} & B & 73.08 & 72.13 & 71.48 & 70.80 & 69.95 & 69.17 & 68.68 & 68.47 & 67.80 \\
    & N & - & 29.60 & 26.40 & 21.93 & 21.65 & 22.36 & 22.03 & 21.63 & 21.00 \\
    & W & 73.08 & 68.86 & 65.04 & 61.03 & 57.88 & 55.40 & 53.13 & 51.21 & 47.08 \\
    \midrule
    \multirow{3}{*}{Fact~(\citeyear{zhou2022forward})} & B & 78.22 & 75.25 & 74.47 & 73.83 & 72.98 & 72.02 & 71.58 & 71.37 & 70.73 \\
    & N & - & 32.80 & 29.40 & 25.20 & 22.30 & 22.44 & 22.67 & 21.77 & 21.45 \\
    & W & 78.22 & 71.99 & 68.03 & 64.11 & 60.31 & 57.44 & 55.28 & 53.10 & 51.02 \\
    \bottomrule
    \end{tabular}
\end{table}


==> table/cifar_switch_perf.tex <==
\begin{table}[t]
\footnotesize
    \centering
    \caption{Base, novel, and weighted performance according to the switch epoch ($E_s$) of updating $h_i \rightarrow \{h_{-i}, h_{i}\}$ on CIFAR100. The values 0 and 100 of $E_s$ indicate $\{h_{-i}, h_{i}\}$ and $h_{i}$, respectively.}\label{tab:cifar_switch}
    \begin{tabular}{ccccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Performance} & \multirow{2}{*}{\vspace{-3pt}$E_s$} & \multicolumn{9}{c}{Session} \\
    \cmidrule{3-11}
    & & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
    \midrule
    \multirow{5}{*}{Base}     & 0   & 65.93 & 52.23 & 50.90 & 49.62 & 52.60 & 48.07 & 48.93 & 50.63 & 48.97 \\
                              & 25  & 65.93 & 53.92 & 51.98 & 51.17 & 53.23 & 49.72 & 49.62 & 51.92 & 50.65 \\
                              & 50  & 65.93 & 54.37 & 51.42 & 50.07 & 51.90 & 48.17 & 48.28 & 50.47 & 48.50 \\
                              & 75  & 65.93 & 54.55 & 50.10 & 47.65 & 48.98 & 45.05 & 44.60 & 45.88 & 43.47 \\
                              & 100 & 65.93 & 51.75 & 45.45 & 41.45 & 38.85 & 34.72 & 33.43 & 32.40 & 29.02 \\
    \midrule
    \multirow{5}{*}{Novel}    & 0   & - & 60.40 & 25.70 & 21.13 & 12.60 & 12.40 & 9.30 & 9.14 & 9.87 \\
                              & 25  & - & 58.20 & 25.30 & 20.53 & 12.10 & 13.28 & 8.97 & 9.00 & 10.10 \\
                              & 50  & - & 57.60 & 27.50 & 23.87 & 13.45 & 15.44 & 11.43 & 10.86 & 12.72 \\
                              & 75  & - & 56.60 & 34.70 & 29.40 & 20.70 & 21.48 & 16.63 & 17.74 & 18.25 \\
                              & 100 & - & 62.20 & 43.10 & 37.80 & 31.15 & 30.48 & 25.90 & 25.71 & 27.17 \\
    \midrule
    \multirow{5}{*}{Weighted} & 0   & 65.93 & 52.86 & 47.30 & 43.92 & 42.60 & 37.58 & 35.72 & 35.35 & 33.33 \\
                              & 25  & 65.93 & 54.25 & 48.17 & 45.04 & 42.95 & 39.00 & 36.07 & 36.11 & 34.43 \\
                              & 50  & 65.93 & 54.62 & 48.00 & 44.83 & 42.29 & 38.54 & 36.00 & 35.87 & 34.19 \\
                              & 75  & 65.93 & 54.71 & 47.90 & 44.00 & 41.91 & 38.12 & 35.28 & 35.52 & 33.38 \\
                              & 100 & 65.93 & 52.55 & 45.11 & 40.72 & 36.92 & 33.47 & 30.92 & 29.94 & 28.28 \\
    \bottomrule
    \end{tabular}
\end{table}





% 체쿠용도
% \begin{table}[t]
% \footnotesize
%     \centering
%     \caption{Base, novel, and weighted performance according to the switch epoch ($E_s$) of updating $\{h_{-i}, h_{i}\} \rightarrow h_i$ on CIFAR100. The values 0 and 100 of $E_s$ indicate $\{h_{-i}, h_{i}\}$ and $h_{i}$, respectively.}\label{tab:cifar_switch}
%     \begin{tabular}{ccccccccccc}
%     \toprule
%     \multirow{2}{*}{Performance} & \multirow{2}{*}{$E_s$} & \multicolumn{9}{c}{Session} \\
%     \cmidrule{3-11}
%     & & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
%     \midrule
%     \multirow{3}{*}{Base}     & 25  & 65.93 & 53.92 & 50.92 & 48.72 & 50.30 & 46.35 & 45.83 & 47.18 & 44.87 \\
%                               & 50  & 65.93 & 54.37 & 52.68 & 51.58 & 53.50 & 49.85 & 49.67 & 51.73 & 50.28 \\
%                               & 75  & 65.93 & 54.55 & 53.10 & 52.62 & 54.33 & 51.10 & 51.07 & 53.22 & 52.28 \\
%     \midrule
%     \multirow{3}{*}{Novel}    & 25  & - & 58.20 & 32.00 & 28.07 & 17.85 & 18.84 & 15.03 & 15.34 & 16.60 \\
%                               & 50  & - & 57.60 & 25.00 & 21.73 & 12.60 & 13.76 & 10.03 & 9.51 & 11.10 \\
%                               & 75  & - & 56.60 & 23.70 & 19.33 & 11.80 & 12.32 & 8.47 & 8.80 & 9.35 \\
%     \midrule
%     \multirow{3}{*}{Weighted} & 25  & 65.93 & 54.25 & 48.21 & 44.59 & 42.19 & 38.26 & 35.57 & 35.45 & 33.56 \\
%                               & 50  & 65.93 & 54.62 & 48.73 & 45.61 & 43.27 & 39.24 & 36.46 & 36.18 & 34.61 \\
%                               & 75  & 65.93 & 54.71 & 48.90 & 45.96 & 43.70 & 39.69 & 36.87 & 36.85 & 35.11 \\
%     \bottomrule
%     \end{tabular}
% \end{table}

==> table/cub_decomp_perf.tex <==
\begin{table}[h]
\footnotesize
    \centering
    \caption{Base, novel, and weighted performance according to the update parts during novel sessions on CUB. Decomposed parameters are described in Table~\ref{tab:notation}.}\label{tab:cub_decomp}
    \vspace{-5pt}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|cccc|ccccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Performance} & \multicolumn{4}{c|}{Update parts} & \multicolumn{11}{c}{Session} \\
    \cmidrule{2-16}
    & $f$ & $h_0$ & $h_{-i}$ & $h_i$ & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
    \midrule
    \multirow{5}{*}{Base} &  &  &  &                    & 69.68 & 69.68 & 69.68 & 69.68 & 69.68 & 69.68 & 69.68 & 69.68 & 69.68 & 69.68 & 69.68 \\
    &  &  &  & \checkmark                               & 69.68 & 58.88 & 55.38 & 51.65 & 46.09 & 44.21 & 42.61 & 41.67 & 41.09 & 40.72 & 39.93 \\
    &  &  & \checkmark & \checkmark                     & 69.68 & 58.88 & 63.41 & 64.20 & 60.57 & 61.39 & 62.61 & 62.72 & 61.80 & 61.20 & 61.82 \\
    &  & \checkmark & \checkmark & \checkmark           & 69.68 & 58.30 & 61.67 & 61.80 & 55.58 & 54.03 & 56.26 & 54.80 & 53.19 & 50.32 & 49.63 \\
    % & \checkmark &  &  & \checkmark                     & 69.16 & 54.96 & 45.62 & 42.80 & 45.83 & 34.12 & 19.88 & 7.69 & 1.03 & 1.07 & 0.14 \\
    % & \checkmark &  & \checkmark & \checkmark           & 69.16 & 54.96 & 48.52 & 40.59 & 37.76 & 31.74 & 26.78 & 21.90 & 23.95 & 17.65 & 19.93 \\
    & \checkmark & \checkmark & \checkmark & \checkmark & 69.68 & 31.04 & 17.51 & 10.95 & 14.13 & 5.83 & 5.54 & 2.62 & 2.69 & 1.28 & 1.41 \\
    \midrule
    \multirow{5}{*}{Novel} &  &  &  &                   & - & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    &  &  &  & \checkmark                               & - & 48.81 & 37.70 & 19.32 & 20.55 & 15.76 & 19.37 & 17.70 & 14.98 & 15.72 & 14.99 \\
    &  &  & \checkmark & \checkmark                     & - & 48.81 & 20.46 & 9.30 & 13.87 & 8.69 & 6.89 & 4.28 & 6.49 & 5.94 & 4.46 \\
    &  & \checkmark & \checkmark & \checkmark           & - & 57.36 & 25.25 & 11.67 & 16.77 & 10.12 & 8.20 & 5.23 & 5.48 & 7.32 & 5.32 \\
    % & \checkmark &  &  & \checkmark                     & - & 59.41 & 32.37 & 18.27 & 20.12 & 15.86 & 9.11 & 5.91 & 1.84 & 2.85 & 1.70 \\
    % & \checkmark &  & \checkmark & \checkmark           & - & 59.41 & 18.71 & 9.97 & 16.33 & 10.36 & 5.86 & 4.96 & 6.88 & 6.37 & 5.21 \\
    & \checkmark & \checkmark & \checkmark & \checkmark & - & 53.42 & 16.24 & 8.74 & 12.15 & 9.05 & 4.92 & 3.10 & 2.52 & 5.89 & 4.40 \\
    \midrule
    \multirow{5}{*}{Weighted} &  &  &  &                & 69.68 & 62.25 & 56.91 & 52.42 & 48.59 & 45.27 & 42.38 & 39.84 & 37.58 & 36.22 & 34.34 \\
    &  &  &  & \checkmark                               & 69.68 & 57.50 & 51.93 & 43.20 & 38.21 & 34.27 & 33.57 & 31.45 & 29.06 & 28.73 & 27.34 \\
    &  &  & \checkmark & \checkmark                     & 69.68 & 57.50 & 55.64 & 50.62 & 46.67 & 43.07 & 40.89 & 37.74 & 36.40 & 34.73 & 32.79 \\
    &  & \checkmark & \checkmark & \checkmark           & 69.68 & 57.89 & 55.15 & 49.47 & 44.15 & 38.88 & 37.66 & 33.70 & 31.36 & 29.83 & 27.28 \\
    % & \checkmark &  &  & \checkmark                     & 69.16 & 55.27 & 43.16 & 37.11 & 38.45 & 27.97 & 15.83 & 7.06 & 1.43 & 1.96 & 0.95 \\
    % & \checkmark &  & \checkmark & \checkmark           & 69.16 & 55.27 & 43.43 & 33.31 & 31.54 & 24.40 & 18.67 & 14.70 & 16.17 & 12.29 & 12.52 \\
    & \checkmark & \checkmark & \checkmark & \checkmark & 69.68 & 33.01 & 17.53 & 10.62 & 13.66 & 7.04 & 5.37 & 2.88 & 2.66 & 3.55 & 2.98 \\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> table/cub_existing_perf.tex <==
\begin{table}[h]
\footnotesize
    \centering
    \caption{Base, novel, and weighted performance of existing algorithms on CUB200. B, N, and W indicate base, novel, and weighted performance, respectively.}\label{tab:cub_existing}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc|ccccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Algorithm} & \multirow{2}{*}{\vspace{-3pt}Perf.} & \multicolumn{9}{c}{Session} \\
    \cmidrule{3-13}
    & & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
    \midrule
    \multirow{3}{*}{Fine-tuning} & B & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & N & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & W & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \midrule
    \multirow{3}{*}{TOPIC~(\citeyear{tao2020few})} & B & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & N & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & W & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \midrule
    \multirow{3}{*}{F2M~(\citeyear{shi2021overcoming})} & B & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & N & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & W & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \midrule
    \multirow{3}{*}{CEC~(\citeyear{zhang2021few})} & B & 75.68 & 74.20 & 73.84 & 73.54 & 72.61 & 72.23 & 71.75 & 71.19 & 71.12 & 70.78 & 70.61\\
    & N & - & 49.35 & 43.67 & 32.65 & 38.80 & 32.11 & 35.12 & 34.16 & 35.16 & 34.51 & 33.96\\
    & W & 75.68 & 71.77 & 68.43 & 63.39 & 62.48 & 58.22 & 57.47 & 55.39 & 54.62 & 53.41 & 52.07\\
    \midrule
    \multirow{3}{*}{Fact~(\citeyear{zhou2022forward})} & B & 77.53 & 75.69 & 75.45 & 75.45 & 75.03 & 74.81 & 74.39 & 74.15 & 74.01 & 73.70 & 73.56\\
    & N & - & 60.09 & 50.24 & 38.55 & 43.68 & 38.59 & 41.20 & 40.55 & 39.89 & 40.41 & 40.38\\
    & W & 77.53 & 73.80 & 70.46 & 65.79 & 65.13 & 61.68 & 61.00 & 59.39 & 57.94 & 57.37 & 56.41\\
    \bottomrule
    \end{tabular}
    }
\end{table}


==> table/cub_switch_perf.tex <==
\begin{table}[h]
\footnotesize
    \centering
    \caption{Base, novel, and weighted performance according to the switch epoch ($E_s$) of updating $h_i \rightarrow \{h_{-i}, h_{i}\}$ on CUB.}\label{tab:cub_switch}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{ccccccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Performance} & \multirow{2}{*}{\vspace{-3pt}$E_s$} & \multicolumn{11}{c}{Session} \\
    \cmidrule{3-13}
    & & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
    \midrule
    \multirow{5}{*}{Base}     & 0   & 69.16 & 61.57 & 59.97 & 57.13 & 59.91 & 62.20 & 55.48 & 54.39 & 56.36 & 59.72 & 61.42 \\
                              & 25  & \\
                              & 50  & \\
                              & 75  & \\
                              & 100 & 69.16 & 61.57 & 53.03 & 46.53 & 48.70 & 46.67 & 38.24 & 35.97 & 37.27 & 43.07 & 44.10 \\
    \midrule
    \multirow{5}{*}{Novel}    & 0   & - & 56.99 & 19.57 & 9.89 & 14.15 & 9.56 & 8.21 & 5.05 & 6.08 & 6.64 & 4.65 \\
                              & 25  & \\
                              & 50  & \\
                              & 75  & \\
                              & 100 & - & 56.99 & 37.44 & 23.05 & 19.21 & 15.35 & 13.33 & 10.97 & 10.77 & 11.92 & 9.90 \\
    \midrule
    \multirow{5}{*}{Weighted} & 0   & 69.16 & 61.08 & 52.94 & 45.76 & 46.24 & 43.91 & 37.17 & 33.36 & 33.30 & 34.37 & 32.71 \\
                              & 25  & \\
                              & 50  & \\
                              & 75  & \\
                              & 100 & 69.16 & 61.08 & 49.95 & 40.59 & 39.39 & 35.87 & 28.48 & 25.22 & 24.98 & 28.05 & 26.85 \\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> table/mini_decomp_perf.tex <==
\begin{table}[h]
\footnotesize
    \centering
    \caption{Base, novel, and weighted performance according to the update parts during novel sessions on miniImageNet. Decomposed parameters are described in Table~\ref{tab:notation}.}\label{tab:mini_decomp}
    \vspace{-5pt}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|cccc|ccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Performance} & \multicolumn{4}{c|}{Update parts} & \multicolumn{9}{c}{Session} \\
    \cmidrule{2-14}
    & $f$ & $h_0$ & $h_{-i}$ & $h_i$ & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
    \midrule
    \multirow{5}{*}{Base} &  &  &  &                    & 73.27 & 73.27 & 73.27 & 73.27 & 73.27 & 73.27 & 73.27 & 73.27 & 73.27 \\
    &  &  &  & \checkmark                               & 73.27 & 67.95 & 63.27 & 60.25 & 59.13 & 57.68 & 55.68 & 53.95 & 52.97 \\
    &  &  & \checkmark & \checkmark                     & 73.27 & 67.95 & 65.67 & 65.25 & 67.17 & 66.67 & 65.38 & 65.12 & 66.88 \\
    &  & \checkmark & \checkmark & \checkmark           & 73.27 & 66.73 & 63.37 & 60.32 & 61.37 & 60.80 & 57.42 & 56.02 & 56.75 \\
    % & \checkmark &  &  & \checkmark                     & 55.55 & 18.93 & 10.40 & 6.47 & 4.97 & 2.78 & 1.93 & 2.85 & 1.12 \\
    % & \checkmark &  & \checkmark & \checkmark           & 55.55 & 18.93 & 11.35 & 6.33 & 4.50 & 2.40 & 1.67 & 2.23 & 0.82 \\
    & \checkmark & \checkmark & \checkmark & \checkmark & 73.27 & 42.68 & 30.10 & 19.80 & 13.43 & 7.72 & 7.85 & 11.23 & 8.15 \\
    \midrule
    \multirow{5}{*}{Novel} &  &  &  &                   & - & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    &  &  &  & \checkmark                               & - & 35.60 & 34.10 & 35.67 & 33.85 & 29.16 & 25.77 & 26.40 & 27.52 \\
    &  &  & \checkmark & \checkmark                     & - & 35.60 & 26.70 & 18.33 & 13.55 & 10.20 & 8.77 & 8.74 & 9.12 \\
    &  & \checkmark & \checkmark & \checkmark           & - & 40.60 & 32.50 & 24.53 & 15.80 & 14.12 & 11.60 & 11.31 & 11.37 \\
    % & \checkmark &  &  & \checkmark                     & - & 36.60 & 29.20 & 27.93 & 23.90 & 22.04 & 14.80 & 11.86 & 8.52 \\
    % & \checkmark &  & \checkmark & \checkmark           & - & 36.60 & 27.30 & 23.33 & 16.35 & 13.40 & 9.67 & 8.26 & 7.62 \\
    & \checkmark & \checkmark & \checkmark & \checkmark & - & 45.60 & 31.60 & 25.80 & 16.20 & 13.72 & 10.90 & 10.37 & 7.97 \\
    \midrule
    \multirow{5}{*}{Weighted} &  &  &  &                & 73.27 & 67.63 & 62.80 & 58.61 & 54.95 & 51.72 & 48.84 & 46.27 & 43.96 \\
    &  &  &  & \checkmark                               & 73.27 & 65.46 & 59.10 & 55.33 & 52.81 & 49.29 & 45.71 & 43.80 & 42.79 \\
    &  &  & \checkmark & \checkmark                     & 73.27 & 65.46 & 60.10 & 55.87 & 53.76 & 50.06 & 46.51 & 44.35 & 43.78 \\
    &  & \checkmark & \checkmark & \checkmark           & 73.27 & 64.72 & 58.96 & 53.16 & 49.97 & 47.07 & 42.14 & 39.55 & 38.60 \\
    % & \checkmark &  &  & \checkmark                     & 55.55 & 20.29 & 13.09 & 10.76 & 9.70 & 8.45 & 6.22 & 6.17 & 4.08 \\
    % & \checkmark &  & \checkmark & \checkmark           & 55.55 & 20.29 & 13.63 & 9.73 & 7.46 & 5.64 & 4.33 & 4.45 & 3.54 \\
    & \checkmark & \checkmark & \checkmark & \checkmark & 73.27 & 42.91 & 30.31 & 21.00 & 14.12 & 9.48 & 8.87 & 10.92 & 8.08 \\
    \bottomrule
    \end{tabular}
    }
\end{table}

==> table/mini_existing_perf.tex <==
\begin{table}[h]
\footnotesize
    \centering
    \caption{Base, novel, and weighted performance of existing algorithms on miniImageNet. B, N, and W indicate base, novel, and weighted performance, respectively.}\label{tab:mini_existing}
    \begin{tabular}{cc|ccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Algorithm} & \multirow{2}{*}{\vspace{-3pt}Perf.} & \multicolumn{9}{c}{Session} \\
    \cmidrule{3-11}
    & & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
    \midrule
    \multirow{3}{*}{Fine-tuning} & B & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & N & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & W & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \midrule
    \multirow{3}{*}{TOPIC~(\citeyear{tao2020few})} 
    & B & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & N & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & W & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \midrule
    \multirow{3}{*}{F2M~(\citeyear{shi2021overcoming})} & B & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & N & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    & W & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    \midrule
    \multirow{3}{*}{CEC~(\citeyear{zhang2021few})} 
    & B & 72.15 & 70.83 & 70.08 & 69.62 & 69.28 & 68.93 & 68.63 & 68.13 & 67.82 \\
    & N & - & 21.40 & 21.00 & 19.60 & 19.80 & 17.84 & 16.93 & 17.37 & 17.42 \\
    & W & 72.15 & 67.03 & 63.07 & 59.61 & 56.91 & 53.91 & 51.40 & 49.43 & 47.66\\
    \midrule
    \multirow{3}{*}{Fact~(\citeyear{zhou2022forward})} 
    & B & 74.98 & 74.62 & 74.28 & 73.85 & 73.62 & 73.37 & 73.08 & 72.85 & 72.67 \\
    & N & - & 14.8 & 13.8 & 13.4 & 13.05 & 12.52 & 11.30 & 12.26 & 12.17 \\
    & W & 74.98 & 70.02 & 65.64 & 61.76 & 58.48 & 55.47 & 52.49 & 50.53 & 48.47 \\
    \bottomrule
    \end{tabular}
\end{table}


==> table/mini_switch_perf.tex <==
\begin{table}[h]
\footnotesize
    \centering
    \caption{Base, novel, and weighted performance according to the switch epoch ($E_s$) of updating $h_i \rightarrow \{h_{-i}, h_{i}\}$ on miniImageNet.}\label{tab:mini_switch}
    \begin{tabular}{ccccccccccc}
    \toprule
    \multirow{2}{*}{\vspace{-3pt}Performance} & \multirow{2}{*}{\vspace{-3pt}$E_s$} & \multicolumn{9}{c}{Session} \\
    \cmidrule{3-11}
    & & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
    \midrule
    \multirow{5}{*}{Base}     & 0   & 55.55 & 43.88 & 43.23 & 42.08 & 43.27 & 43.18 & 46.12 & 44.93 & 42.25 \\
                              & 25  & \\
                              & 50  & \\
                              & 75  & \\
                              & 100 & 55.55 & 43.88 & 41.97 & 39.95 & 40.25 & 39.20 & 41.97 & 40.87 & 37.10 \\
    \midrule
    \multirow{5}{*}{Novel}    & 0   & - & 22.40 & 17.20 & 13.67 & 7.00 & 6.24 & 5.87 & 5.17 & 4.98 \\
                              & 25  & \\
                              & 50  & \\
                              & 75  & \\
                              & 100 & - & 22.40 & 20.80 & 22.27 & 16.9 & 15.68 & 13.90 & 11.09 & 8.00 \\
    \midrule
    \multirow{5}{*}{Weighted} & 0   & 55.55 & 42.23 & 39.51 & 36.40 & 34.20 & 32.32 & 32.70 & 30.28 & 27.34 \\
                              & 25  & \\
                              & 50  & \\
                              & 75  & \\
                              & 100 & 55.55 & 42.23 & 38.94 & 36.41 & 34.41 & 32.28 & 32.61 & 29.89 & 25.46 \\
    \bottomrule
    \end{tabular}
\end{table}
